Expanding Perspectives on Data Privacy: Insights from Rural Togo

Passively collected "big" data sources are increasingly used to inform critical development policy decisions in low- and middle-income countries. While prior work highlights how such approaches may reveal sensitive information, enable surveillance, and centralize power, less is known about the corresponding privacy concerns, hopes, and fears of the people directly impacted by these policies -- people sometimes referred to as experiential experts. To understand the perspectives of experiential experts, we conducted semi-structured interviews with people living in rural villages in Togo shortly after an entirely digital cash transfer program was launched that used machine learning and mobile phone metadata to determine program eligibility. This paper documents participants' privacy concerns surrounding the introduction of big data approaches in development policy. We find that the privacy concerns of our experiential experts differ from those raised by privacy and development domain experts. To facilitate a more robust and constructive account of privacy, we discuss implications for policies and designs that take seriously the privacy concerns raised by both experiential experts and domain experts.

==> sections/participants_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\scriptsize
\begin{longtable}{@{}lllllllllll@{}}
\caption{Interview participants, labeled with participant ID and pseudonym. Names in Togo are often associated with a particular gender and religious or ethnic group. All pseudonyms were developed by the second author to align with the gender and religious or ethnic group of the participant's real name. NA (not asked) in the Novissi status and education columns indicates that the participant was not asked the question. NR (no response) in the age column indicates that the participant did not respond to the question.} \\
 

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\toprule
\textbf{ID} & \textbf{Pseudonym} & \textbf{Gender} & \textbf{Age} & \textbf{Ethnicity}  & \textbf{Religion} & \textbf{Novissi status} & \textbf{Education} & \textbf{Occupation}      & \textbf{Interview guide}    & \textbf{Interview language} \\ \midrule
\multicolumn{11}{l}{\textit{Panel A: Pilot Phase 1: phone interviews}}                                                                                                                                                                                     \\
P01         & Welyh              & Female          & 34           & Lamba               & Christian         & Beneficiary             & Priamry school     & Hairdresser              & Combined pilot              & French                      \\
P02         & Tiguidame          & Female          & 52           & Moba                & Christian         & Beneficiary             & Primary school     & Farmer                   & Combined pilot              & French                      \\
P03         & Toubonoh           & Male            & 39           & Lamba               & Muslim            & Registered              & Middle school      & Veterinarian             & Combined pilot              & French                      \\
P04         & Sodou              & Male            & 27           & Gangan              & Animist           & Registered              & High school        & Farmer                   & Combined pilot              & French                      \\
P05         & Gnimda             & Female          & 28           & Fon                 & Christian         & Unregistered            & High school        & Market seller            & Combined pilot              & French                      \\
P06         & Akpedje            & Female          & 37           & Akebou              & Christian         & Unregistered            & High school        & Delivers babies          & Combined pilot              & French                      \\
P07         & Akpene             & Female          & 46           & Akposso             & Christian         & Unregistered            & Middle school      & Farmer                   & Combined pilot              & Ewe                         \\
P08         & Kokouvi            & Male            & 32           & Kabyé               & Christian         & Unregistered            & High school        & Animal husbandry         & Combined pilot              & French                      \\
P09         & Etsè               & Male            & 52           & Ewe        & Christian         & Registered              & High school        & Clothing designer        & Combined pilot              & French                      \\
P10         & Kibalo             & Male            & 34           & Laffa               & Christian         & Unregistered            & High school        & Farmer                   & Combined pilot              & Kabyé                       \\
P11         & Douti              & Male            & 72           & Moba                & Catholic          & Beneficiary             & None               & Shephard, farmer         & Combined pilot              & French                      \\
P12         & Ismael             & Male            & 22           & Kotokoli   & Muslim            & Beneficiary             & Primary school     & Farmer                   & Combined pilot              & Kotokoli                    \\
P13         & Assibi             & Female          & 41           & Moba                & Christian         & Beneficary              & Primary school     & Selling local beer       & Combined pilot              & French                      \\
P14         & Sebabi             & Female          & 50           & Kabyé               & None              & Registered              & Primary school     & Farmer                   & Combined pilot              & Kotokoli                    \\
P15         & Amina              & Female          & NR           & Peule               & Muslim            & Beneficiary             & Middle school      & Farmer, sells firewood   & Combined pilot              & Kotokoli                    \\
P16         & Akouvi             & Female          & 19           & Ewe            & Christian         & Registered              & High school        & Baker of breads          & Combined pilot              & Ewe                         \\
\multicolumn{11}{l}{\textit{Panel B: Pilot Phase 2: fieldwork - village 1}}                                                                                                                                                                                \\
P17         & Pawoulassim        & Male            & 45           & Kabyé               & None              & Registered              & High school        & Farmer and fisher        & Social protection pilot     & Kabyé                       \\
P18         & Leleng             & Female          & 70           & Kabyé               & None              & Beneficiary             & NA                 & Nothing                  & Social protection pilot     & Kabyé                       \\
P19         & Magnoudewa         & Female          & 29           & Kabyé               & Protestant        & NA                      & Middle school      & Tailor and sells food    & Data privacy pilot          & Kabyé                       \\
P20         & Pidenam            & Male            & 32           & Kabyé               & Pagan             & NA                      & High school        & CVD                      & Social protection pilot     & Kabyé                       \\
P21         & Birewa             & Male            & 42           & Kabyé               & Catholic          & NA                      & None               & Farmer                   & Social protection pilot     & Kabyé                       \\
P22         & Patouani           & Male            & 32           & Kabyé               & Protestant        & NA                      & High school        & CVD                      & Social protection pilot     & Kabyé                       \\
P23         & Samtou             & Male            & 39           & Kabyé               & Pagan             & NA                      & Primary school     & Farmer                   & Social protection pilot     & Kabyé                       \\
P24         & Ewenam             & Female          & 52           & Kabyé               & Pagan             & NA                      & Primary school     & Farmer                   & Social protection pilot     & Kabyé                       \\
P25         & Lidaw              & Female          & 60           & Kabyé               & Protestant        & NA                      & None               & Farmer                   & Social protection pilot     & Kabyé                       \\
\multicolumn{11}{l}{\textit{Panel C: Pilot Phase 2: fieldwork - village 2}}                                                                                                                                                                                \\
P26         & Mèhèza             & Female          & 50           & Ewe                 & Christian         & NA                      & None               & Farmer                   & Data privacy pilot          & Ewe                         \\
P27         & Dzodzina           & Female          & 25           & Ewe                 & Christian         & NA                      & Middle school      & Market seller, farmer    & Data privacy pilot          & Ewe                         \\
P28         & Apedo              & Male            & 30           & Ewe                 & Christian         & NA                      & High school        & Farmer                   & Data privacy pilot          & Ewe                         \\
P29         & Agbeko             & Male            & 70           & Ewe                 & Christian         & NA                      & Middle school      & Farmer and tailor        & Data privacy pilot          & Ewe                         \\
P30         & Kafui              & Female          & 24           & Ewe                 & Christian         & NA                      & Middle school      & Artisian                 & Social protection pilot     & Ewe                         \\
P31         & Etonam             & Female          & 30           & Ewe                 & Christian         & NA                      & Primary school     & Farmer                   & Social protection pilot     & Ewe                         \\
P32         & Yonam              & Female          & 27           & Ewe        & Christian         & NA                      & High school        & Market seller            & Social protection pilot     & Ewe                         \\
P33         & Sika               & Female          & 25           & Ewe                 & Christian         & NA                      & High school        & Tailor                   & Social protection pilot     & Ewe                         \\
P34         & Ablavi             & Female          & 33           & Ewe                 & Christian         & NA                      & None               & Farmer                   & Social protection pilot     & Ewe                         \\
P35         & Elom               & Male            & 52           & Ewe                 & Christian         & NA                      & None               & Farmer                   & Data privacy pilot          & Ewe                         \\
P36         & Assou              & Male            & 25           & Ewe                 & Christian         & NA                      & None               & Artisian, farmer         & Data privacy pilot          & Ewe                         \\
\multicolumn{11}{l}{\textit{Panel D: Fieldwork - village 1}}                                                                                                                                                                                      \\
P37         & Toï                & Male            & 34           & Kabyé               & Animist           & Beneficiary             & High school        & Farmer                   & Social protection           & Kabyé                       \\
P38         & Essozinam          & Male            & 42           & Kabyé               & Animist           & Beneficiary             & High school        & Farmer                   & Social protection           & Kabyé                       \\
P39         & Kibangbene         & Male            & 60           & Kabyé               & Animist           & Beneficiary             & Middle school      & Farmer                   & Social protection           & Kabyé                       \\
P40         & Mazamaesso         & Female          & 27           & Kabyé               & Christian         & Registered              & Middle school      & Palm oil producer        & Data privacy part 1         & Kabyé                       \\
P41         & Kibanou            & Male            & 43           & Kabyé               & Christian         & Registered              & Middle school      & Farmer                   & Data privacy part 1         & Kabyé                       \\
P42         & Maha               & Male            & 56           & Kabyé               & Animist           & Beneficiary             & None               & Farmer                   & Data privacy part 1         & Kabyé                       \\
P43         & Meyebinesso        & Female          & 64           & Kabyé               & Christian         & Beneficiary             & Primary school     & Seller                   & Data privacy part 1         & Kabyé                       \\
P44         & Badowe             & Male            & 45           & Kabyé               & Animist           & Beneficiary             & Middle school      & Farmer                   & Social protection           & Kabyé                       \\
P45         & Mangelewe          & Female          & 39           & Kabyé               & Christian         & Registered              & Primary school     & Farmer                   & Social protection           & Kabyé                       \\
P46         & Tchaa              & Male            & 45           & Kabyé               & Animist           & Beneficiary             & None               & Farmer                   & Social protection           & Kabyé                       \\
P47         & Kobyo              & Male            & 64           & Kabyé               & Christian         & Beneficiary             & High school        & Farmer                   & Social protection           & Kabyé and French              \\
P48         & Hezu               & Male            & 35           & Kabyé               & Animist           & Beneficiary             & Middle school      & Farmer                   & Social protection           & Kabyé                       \\
P49         & Cilabalo           & Male            & 51           & Kabyé               & Christian         & Registered              & High school        & Farmer                   & Social protection           & Kabyé                       \\
P50         & Kemeyabalo         & Male            & 30           & Kabyé               & Christian         & Registered              & High school        & Farmer                   & Social protection           & Kabyé                       \\
P51         & Kujukalo           & Female          & 74           & Kabyé               & Christian         & Registered              & None               & Farmer                   & Social protection           & Kabyé                       \\
P52         & Telu               & Male            & 25           & Kabyé               & Christian         & Registered              & Middle school      & Farmer                   & Social protection           & Kabyé                       \\
P53         & Soka               & Female          & 40           & Kabyé               & Christian         & Registered              & Primary school     & Farmer                   & Data privacy part 1, 2, 3         & Kabyé                       \\
P54         & Keziye             & Male            & 40           & Kabyé               & Animist           & Beneficiary             & Middle school      & Farmer                   & Data privacy part 1         & Kabyé                       \\
P55         & Bilim              & Male            & 55           & Kabyé               & Christian         & Beneficiary             & Primary school     & Farmer, meat seller      & Data privacy part 1, 2, 3         & Kabyé                       \\
P56         & Naka               & Female          & 30           & Kabyé               & Christian         & Registered              & Middle school      & Farmer, seller           & Data privacy part 1, 2, 3         & Kabyé                       \\
P57         & Nèmè               & Female          & 40           & Kabyé               & Christian         & Unregistered            & None               & Seller                   & Social protection           & Kabyé                       \\
P58         & Tonga              & Female          & 33           & Kabyé               & Christian         & Registered              & Middle school      & Farmer                   & Data privacy part 1, 2, 3         & Kabyé                       \\
P59         & Essodina           & Female          & NR           & Kabyé               & Animist           & Registered              & None               & Farmer, seller           & Social protection           & Kabyé                       \\
P60         & Sama               & Male            & 65           & Kabyé               & Animist           & Beneficiary             & Middle school      & Farmer                   & Social protection           & Kabyé                       \\
P61         & Soka               & Male            & 25           & Kabyé               & Christian         & Registered              & Middle school      & Roofing work             & Key informat & Kabyé                       \\
P62         & Padayodi           & Female          & 30           & Kabyé               & None              & Registered              & None               & Farmer, seller           & Data privacy part 1, 2, 3         & Kabyé                       \\
P63         & Kpatcha            & Male            & 70           & Kabyé               & Animist           & Beneficiary             & None               & Farmer                   & Social protection           & Kabyé                       \\
\multicolumn{11}{l}{\textit{Panel E: Fieldwork - village 2}}                                                                                                                                                                                      \\
P64         & Kossiwa            & Female          & 38           & Kabyé               & None              & Beneficiary             & Primary school     & Seller                   & Social protection           & Kabyé                       \\
P65         & Kawo               & Male            & 45           & Kabyé               & Christian         & Beneficiary             & Middle school      & Farmer                   & Social protection           & Kabyé                       \\
P66         & Alfa               & Male            & 48           & Kabyé               & None              & Beneficiary             & Primary school     & Farmer                   & Data privacy part 1         & Kabyé                       \\
P67         & Palakyem           & Male            & 50           & Kabyé               & Catholic          & Beneficiary             & None               & Farmer                   & Data privacy part 1, 2, 3         & Kabyé                       \\
P68         & Badiou             & Male            & 55           & Kotokoli            & Muslim            & Registered              & Primary school     & Farmer                   & Social protection           & Kotokoli                    \\
P69         & Achraf             & Male            & 55           & Kotokoli            & Muslim            & Registered              & Middle school      & Farmer                   & Social protection           & Kotokoli                    \\
P70         & Hamdiya            & Female          & 29           & Kotokoli            & Muslim            & Beneficiary             & Middle school      & Seller                   & Social protection           & Kotokoli                    \\
P71         & Fousseni           & Male            & 27           & Kotokoli            & Muslim            & Beneficiary             & Middle school      & Bricklayer               & Social protection           & Kotokoli                    \\
P72         & Aledjou            & Male            & 23           & Kotokoli            & Muslim            & Registered              & University         & Student                  & Social protection           & Kotokoli                    \\
P73         & Saeeb              & Male            & 32           & Kabyé               & Muslim            & Beneficiary             & Middle school      & Farmer                   & Social protection           & Kabyé                       \\
P74         & Banawe             & Male            & 58           & Kabyé               & Animist           & Beneficiary             & None               & Farmer                   & Social protection           & Kabyé                       \\
P75         & Songhaï            & Male            & 40           & Kotokoli            & Muslim            & Registered              & Primary school     & Farmer                   & Social protection           & Kotokoli                    \\
P76         & Fataou             & Male            & 20           & Peule               & Muslim            & Unregistered            & None               & Farmer                   & Social protection           & Kotokoli                    \\
P77         & Gouni              & Female          & 23           & Kotokoli            & Muslim            & Beneficiary             & Middle school      & Farmer                   & Social protection           & Kotokoli                    \\
P78         & Mohamadou          & Male            & NR           & Peule               & Muslim            & Beneficiary             & None               & Farmer                   & Social protection           & Kotokoli                    \\
P79         & Takiath            & Female          & NR           & Peule               & Muslim            & Beneficiary             & None               & Oil seller               & Social protection           & Kotokoli                    \\
P80         & Mansourath         & Female          & NR           & Peule               & Muslim            & Beneficiary             & None               & Oil seller               & Social protection           & Kotokoli                    \\
P81         & Hadidjatou         & Female          & NR           & Peule               & Muslim            & Beneficiary             & None               & Oil seller               & Social protection           & Kotokoli                    \\
P82         & Mansour            & Male            & NR           & Peule               & Muslim            & Registered              & None               & Farmer                   & Social protection           & Kotokoli                    \\
P83         & Moustapha          & Male            & NR           & Peule               & Muslim            & Beneficiary             & None               & Farmer                   & Social protection           & Kotokoli                    \\
P84         & Sadjida            & Female          & NR           & Kotokoli            & Muslim            & Beneficiary             & None               & Food seller              & Data privacy part 1         & Kotokoli                    \\
P85         & Ahmed              & Male            & 45           & Kotokoli            & Christian         & Beneficary              & High school        & Helps mayor              & Social protection           & Kotokoli and French         \\
P86         & Abide              & Female          & 38           & Kabyé               & Christian         & Beneficiary             & Primary school     & Seller                   & Data privacy part 1         & Kabyé                       \\
P87         & Panawé             & Male            & 55           & Kotokoli            & Muslim            & Beneficiary             & Middle school      & Farmer                   & Data privacy part 1         & Kotokoli                    \\
P88         & Meyebinebè         & Female          & 42           & Kabyé               & Animist           & Unregistered            & None               & Seller                   & Data privacy part 1         & Kabyé                       \\
P89         & Mazalo             & Female          & 65           & Kabyé               & Animist           & Beneficiary             & None               & None                     & Data privacy part 1         & Kabyé                       \\
P90         & Solim              & Male            & 27           & Kabyé               & Muslim            & Beneficiary             & University         & Student at university    & Social protection           & Kabyé, French, English      \\
P91         & Tchilabalo         & Male            & 36           & Kabyé               & Christian         & Beneficiary             & Middle school      & Farmer                   & Data privacy part 1         & Kabyé                       \\
P92         & Tchilalo           & Female          & 28           & Kabyé               & Animist           & Registered              & Middle school      & Tailor                   & Data privacy part 1, 2, 3         & Kabyé and French            \\
P93         & Soumbalo           & Male            & 38           & Kabyé               & Christian         & Beneficiary             & Middle school      & Farmer                   & Data privacy part 1, 2         & Kabyé                       \\
P94         & Awete              & Male            & 46           & Kabyé               & Christian         & Beneficiary             & Middle school      & Retired Civil Servant    & Data privacy part 1, 2, 3         & Kabyé and French            \\
P95         & Adjeki             & Male            & 40           & Kabyé               & None              & Registered              & None               & Farmer                   & Social protection           & Kabyé                       \\
P96         & Essohounam         & Male            & 83           & Kabyé               & Animist           & Registered              & Middle school      & Retired teacher          & Data privacy part 1, 2, 3         & Kabyé and French            \\
P97         & Mazabalo           & Male            & 37           & Kabyé               & Christian         & Beneficary              & Middle school      & Farmer                   & Key informant               & Kabyé                       \\
P98         & Rachid             & Male            & 34           & Peule               & Muslim            & Beneficary              & Middle school      & CVD, farmer              & Key informant               & Kabyé                       \\
P99         & Pyabalou           & Male            & 34           & Kabyé               & Animist           & Beneficiary             & None               & Chief of village, farmer & Key informant               & Kabyé                       \\
P100        & --same as P90--    & -- P90 --       & -- P90 --    & -- P90 --           & -- P90 --         & -- P90 --               & -- P90 --          & -- P90 --                & -- P90 --                   & -- P90 --                   \\
\multicolumn{11}{l}{\textit{Panel F: Fieldwork - village 3}}                                                                                                                                                                                      \\
P101        & Kokou              & Male            & 58           & Ewe                 & Christian         & Registered              & High school        & Mechanic                 & Key informant               & Ewe                         \\
P102        & Abla               & Female          & 55           & Ewe                 & Christian         & Registered              & Primary school     & Farmer                   & Social protection           & Ewe                         \\
P103        & Afivi              & Female          & 37           & Ewe                 & Christian         & Registered              & None               & Farmer                   & Social protection           & Ewe                         \\
P104        & Komi               & Male            & 50           & Ewe & Animist           & Beneficiary             & None               & Farmer                   & Key informant               & Ewe                         \\
P105        & Sogbe              & Male            & 70           & Ewe & Animist           & Unregistered            & None               & Farmer                   & Social protection           & Ewe                         \\
P106        & Etonam             & Female          & 65           & Ewe   & Animist           & Beneficiary             & None               & Farmer                   & Social protection           & Ewe                         \\
P107        & Enyonam            & Female          & 30           & Ewe                 & Christian         & Beneficiary             & None               & Farmer                   & Data privacy part 1         & Ewe                         \\
P108        & Emefa              & Female          & 30           & Ewe          & Animist           & Registered              & Primary school     & Farmer                   & Social protection           & Ewe                         \\
P109        & Djidula            & Male            & 60           & Ewe          & Animist           & Unregistered            & None               & Welder                   & Data privacy part 1, 2, 3         & Ewe                         \\
P110        & Dodzi              & Female          & 70           & Ewe & Christian         & Beneficiary             & Primary school     & Farmer                   & Social protection           & Ewe                         \\
P111        & Senyo              & Male            & 33           & Ewe        & Christian         & Registered              & Middle school      & Driver                   & Data privacy part 1, 2, 3         & Ewe                         \\
P112        & Kekeli             & Female          & 22           & Ewe         & Christian         & Unregistered            & Middle school      & Hairdresser              & Social protection           & Ewe                         \\
P113        & Kossi              & Male            & 29           & Ewe        & Animist           & Registered              & Primary school     & Farmer                   & Social protection           & Ewe                         \\
P114        & Koffi              & Male            & 50           & Ewe        & Animist           & Registered              & Primary school     & Farmer                   & Social protection           & Ewe                         \\
P115        & Abalo              & Male            & 35           & Ewe   & Christian         & Unregistered            & Primary school     & Farmer                   & Data privacy part 1         & Ewe                         \\
P116        & Mawuena            & Male            & 35           & Ewe        & Christian         & Registered              & Middle school      & Farmer                   & Data privacy part 1         & Ewe                         \\
P117        & Ayaba              & Female          & 26           & Ewe          & Christian         & Registered              & High school        & Seller                   & Key informant & Ewe                         \\
P118        & Edem               & Male            & 33           & Ewe   & Animist           & Registered              & Middle school      & Barber                   & Social protection           & Ewe                         \\
P119        & Anoumou            & Male            & 31           & Ewe                 & Christian         & Registered              & Middle school      & Electrician              & Social protection           & Ewe                         \\
P120        & Holali             & Female          & 30           & Ewe                 & Christian         & Registered              & Primary school     & House wife               & Data privacy part 1         & Ewe                         \\
P121        & Mensah             & Male            & NR           & Ewe                 & Animist           & Registered              & None               & Farmer                   & Social protection           & Ewe                         \\
P122        & Dela               & Female          & 30           & Ewe                 & Animist           & Beneficiary             & None               & Farmer                   & Data privacy part 1, 2, 3         & Ewe                         \\
P123        & Anani              & Male            & 60           & Ewe                 & Animist           & Registered              & Middle school      & Welder                   & Data privacy part 1, 2, 3         & Ewe and French              \\
P124        & Kodjo              & Male            & 32           & Kabyé               & Christian         & Unregistered            & Middle school      & Farmer                   & Data privacy part 1, 2         & Ewe                         \\
P125        & Komla              & Male            & 25           & Ewe                 & Christian         & Registered              & Middle school      & Farmer                   & Data privacy part 1         & Ewe                         \\ \bottomrule




\end{longtable}


\normalsize
